Self-supervised learning for radio-astronomy source classification: a benchmark

The upcoming Square Kilometer Array (SKA) telescope marks a significant step forward in radio astronomy, presenting new opportunities and challenges for data analysis. Traditional visual models pretrained on optical photography images may not perform optimally on radio interferometry images, which have distinct visual characteristics. Self-Supervised Learning (SSL) offers a promising approach to address this issue, leveraging the abundant unlabeled data in radio astronomy to train neural networks that learn useful representations from radio images. This study explores the application of SSL to radio astronomy, comparing the performance of SSL-trained models with that of traditional models pretrained on natural images, evaluating the importance of data curation for SSL, and assessing the potential benefits of self-supervision to different domain-specific radio astronomy datasets. Our results indicate that, SSL-trained models achieve significant improvements over the baseline in several downstream tasks, especially in the linear evaluation setting; when the entire backbone is fine-tuned, the benefits of SSL are less evident but still outperform pretraining. These findings suggest that SSL can play a valuable role in efficiently enhancing the analysis of radio astronomical data. The trained models and code is available at: \url{https://github.com/dr4thmos/solo-learn-radio}

==> Chapters/Method_Preproc.tex <==
The scouting of new objects and precise annotatation requires an interactive tweaking of intensity pixel values to highlight various sources details. In usual astronomical image analysis tools as SAOImageDS9\cite{joye2003ds9} and CARTA\cite{comrie2021carta}, a common approach is to stretch the histogram with different functions (e.g. log, asinh, ...), setting an interval (e.g. MinMax, Percentile, Zscale). By fixing the interval to MinMax, and by grouping stretching function in those that squeeze and stretch the histogram we build a 3 channel image that highlights different peculiarity of the sources under inspection (\ref{augmentation}). 
\hl{spiegare quale preprocessing usiamo noi}

==> Chapters/Method_draft.tex <==
\section{Method}
\subsection{Self supervised learning} To ensure a robust and comprehensive benchmark we decided to use \textit{\textbf{solo-learn}} library that implements a wide range of state-of-the-art self-supervised learning methods. Using a single framework ensures that all experiments are implemented with consistent standards, reducing variability and potential biases that might arise from different coding practices. From the plethora of methods available we select a subset of SSL techniques minimizing the overlap within strategies to reach a comprehensive and efficient benchmark. Whereas there is limited research on applying SSL methods to radio astronomy images, to build a solid baseline it's prudent to start with well-established models like CNNs, specifically ResNet, leaving out vision transformers (as ViTs require significantly amount of computational resources and since those can exhibit instability during training). Therefore, methods that principally rely their efficiency on ViT (e.g. MAE or DinoV2) are not considered.

A core technique employed by the considered methods involves generating two augmented views of the same image x’ and x’’. This approach is pivotal in learning robust feature representations, as it enables the model to understand and capture the intrinsic properties of the images through various augmentations.

In SimCLr\cite{chen2020simplesimclr} the views are processed by a model producing representations z’ and z’’. The methods rely on attracting representations of views generated by the same image, while repelling the others. In order to make that, SimCLr use a projection network and a loss defined as:
\[
     \mathcal{L}_{SimCLR} = -\log \frac{\exp(\text{sim}(h_i, h_j) / \tau)}{\sum_{k=1}^{2N} \mathbb{1}_{[k \neq i]} \exp(\text{sim}(h_i, h_k) / \tau)}
     \]
where \( h_i \) and \( h_j \) are the projections of z’ and z’’,   \(\text{sim}\) is the cosine similarity, and \(\tau\)  is a temperature parameter.
Tackling the problem from a slightly different perspective is BYOL, that doesn’t leverage negative examples (repelling). It involves two networks, online and target, and a predictor on top of online projector. The target network is freezed and updates through an EMA each epoch. The pretext tasks is to predict the output of the target network projection:
\[
     \mathcal{L}_{BYOL} = \|q_\theta(z_{\text{online}}) - z_{\text{target}}\|_2^2
     \]
where \( q_\theta \) is the predictor. Starting from BYOL, DINO addresses the problem from a knowledge distillation angle. The loss could be represented as:
\[
     \mathcal{L}_{DINO} = \sum_{i} \text{KL}(\sigma(z_i^t / \tau_t), \sigma(z_i^s / \tau_s))
     \]
where \(z_i^t\) and \(z_i^s\) are the outputs (representations) of the teacher and student networks, respectively, \textit{\textbf{\(\sigma\)}} denotes the softmax function, and \(\tau_t\)and \(\tau_s\) are temperature parameters for the teacher and student networks. DINO uses multi-crop strategy at different resolutions, in order to encourage “local-to-global” correspondences. 
WMSE distinguishes himself by using a whitening operation that maps the representation space into a spherical distribution. The loss could be represented as: uses the mutual information maximization in combination with whitening the representations.
\[
     \mathcal{L}_{WMSE} = \frac{1}{N} \sum_{i=1}^N \| \text{W}(z_i^{(1)}) - \text{W}(z_i^{(2)}) \|_2^2
     \]
where \( z_i^{(1)} \) and \( z_i^{(2)} \) are the representations of two augmentations of the same image, and \(\text{W}(z)\) denotes the whitening transformation applied to representation \( z \).

Clustering is historically one of the most suitable methods for unsupervised analysis. Swapped Assignment between Views (SwAV)\cite{caron2020swav} uses this technique innovatively, assigning pseudo-labels to different views of the same image and comparing the swapped assignments. Instead of performing pairwise comparisons between all features, SwAV matches representations to prototypes updated online. 

SwAV operates on pairs of augmented views (v', v'') of the same image. For each view, it computes a soft assignment q to a set of prototypes C. The key to the method is the 'swapping': the assignment q computed on one view is used to predict the representation of the other view.
The SwAV loss function can be formulated as:
\[
     \mathcal{L}_{\text{SwAV}} = \ell(q', p'') + \ell(q'', p')
\]
where ($\ell$) is the cross-entropy, q' and q'' are the soft assignments for the two views, and p' and p'' are the predicted distributions over the prototypes. This formulation encourages consistency between different views of the same image.

Several methods leverage the concept of nearest neighbors, as NNCLR. A very recent method called All4One\cite{estepa2023all4one}, use that concept in combination with several others, as we could states in the loss function:
 \[
     \mathcal{L}_{All4One} = \lambda_{nn} \mathcal{L}_{nearest\_neighbors} + \lambda_{centr} \mathcal{L}_{centroids} + \lambda_{red} \mathcal{L}_{redundancy}
     \]
     where \( \mathcal{L}_{nn} \) is the loss computed between the NN of the first view and the second view, \( \mathcal{L}_{centroids} \) use a self-attention mechanism to calculate a pair of centroids in the NN of each views, \( \mathcal{L}_{redundancy} \) makes advantage of Barlow Twins principle of redundacy reduction, and \( \lambda_{nn} \), \( \lambda_{centr} \) and \( \lambda_{red} \) are weighting factors.

\subsection{Experimental setup}
The experimental setup is designed as a benchmark, conducting a methodical analysis by altering key parameters to address our inquiries. First we want to asses the impact of introducting an augmentation suited for radio images, as described in section ..., namely $\{A_{\text{naive}}, A_{\text{radio}}\} \in A$. Those augmentations are applied to unlabeled datasets with different compositions and sizes, which are part of our investigation. In particular, one dataset with limited amount of data but with image-centered objects, and another one sequentially cropped from big maps with huge size, are compared, respectively  $\{D_{\text{curated}}, D_{\text{uncurated}}\} \in D$, detailed information could be found in section ... . 
Part of the recipe of self-supervision is to train a model on unlabeled data by using a pretext task. Therefore we consider five different tasks, namely, $\{P_{\text{byol}}, P_{\text{simclr}}, P_{\text{swav}}, P_{\text{dino}}, P_{\text{wmse}}\} \in P$ for a dual scope: finding the best methods to perform downstream tasks in radio image domain, and to study the impact of A and D on specific pretext tasks. 
As additional hyperparameter we studied the impact of using different backbones in the pretext task's architecture, in particular $\{B_{\text{resnet18}}, B_{\text{resnet50}}\} \in B$. By defining $ \Theta $ the set of all combination of hyperparameters $ \{A,D,P,B\} $ and $ f_{\theta} $ a feature extractor trained using a single combination, we need to quantitatively evaluate the performance on multiple downstream tasks $\{T_{\text{mirabest}}, T_{\text{rgz}}, T_{\text{frg}}, T_{\text{msrs}}, T_{\text{vlass}}\} \in T$, which shows different number of classes and different acquisition hardware.
Then, the main measurable goal is to find the best hyperparameters $\theta^*$ that maximise the mean accuracies across all downstream tasks T:
\[ \theta^* = \arg \max_{\theta \in \Theta} \frac{\sum_{t \in T} Acc_{\text{t}}(f_{\theta}(t))}{|T|}  \]

The amount of models produced could be calculated considering $ \Theta $ cardinality as the carthesian product of the hyperparameters $ |\Theta| = |A| \times |D| \times |P| \times |B| = 40 $.
